Interpretable Multi-Headed Attention for Abstractive Summarization at Controllable Lengths

Abstractive summarization at controllable lengths is a challenging task in natural language processing. It is even more challenging for domains where limited training data is available or scenarios in which the length of the summary is not known beforehand. At the same time, when it comes to trusting machine-generated summaries, explaining how a summary was constructed in human-understandable terms may be critical. We propose Multi-level Summarizer (MLS), a supervised method to construct abstractive summaries of a text document at controllable lengths. The key enabler of our method is an interpretable multi-headed attention mechanism that computes attention distribution over an input document using an array of timestep independent semantic kernels. Each kernel optimizes a human-interpretable syntactic or semantic property. Exhaustive experiments on two low-resource datasets in the English language show that MLS outperforms strong baselines by up to 14.70% in the METEOR score. Human evaluation of the summaries also suggests that they capture the key concepts of the document at various length-budgets.

==> related.tex <==
\section{Related Works}\vspace{-0.2cm}

%From handcrafted features to learned models, text summarization has garnered a lot of attention from researchers in recent times. We review some of them in this section.\vspace{0.05cm}

%\textit{Non-budgeted summarization : }A majority of the existing techniques adopt various sampling techniques to construct a balanced summary of the input document. Sentences appearing in the document are sampled with some qualitative optimization objectives to construct a representative summary. One of the earlier efforts following this approach is TextRank~\cite{mihalcea2004textrank}. Assuming a document-graph where each sentence is represented as a node, sentences in the input document are ranked based on their similarity with the neighboring vertices. An extractive summary of the document is then constructed by sampling the vertices with the highest pairwise similarities. Garg et al.~\cite{garg2009clusterrank} extended TextRank by adding a prior clustering step to summarize meeting proceedings. The major limitation of these approaches is that they do not take into account the syntactic and semantic structure of a sentence while computing similarities. Consequently, sentences like “The cat sat on a mat” are considered similar to sentences such as “The mat sat on a cat”.More recently~\cite{narayan2018ranking} and ~\cite{vinyals2015pointer} have shown that this can be addressed by employing a supervised deep neural network to construct extractive summaries. On the other hand, ~\cite{rush2015neural}, ~\cite{nallapati2016abstractive}, and~\cite{see2017get} have shown that human-like capabilities e.g. multi-sentence compression, common knowledge usage~\cite{liu2018toward}, and paraphrasing can also be introduced to construct abstractive summaries using supervised sequence-to-sequence memory networks.\vspace{0.03cm}

\textit{Physical structure: }Some of the early works leveraged the physical structure of the input document to construct summaries at multiple levels. Utilizing the hierarchical DOM-tree structure, Buyukkokten et al.~\cite{buyukkokten2001seeing} identified structural components at different levels using HTML tags which were subsequently used to generate summaries at different budgets. Yang et al.~\cite{yang2003fractal} also leveraged the physical structure of a document to construct summaries for mobile devices. Contrary to these methods, we do not exploit or assume any prior knowledge of the structure of the document.\looseness=-1\vspace{0.02cm} 


%Inspired by the recent success of deep neural networks~\cite{rush2015neural, chopra2016abstractive,vinyals2015pointer,see2017get} for generating balanced summaries at single granularity, we have developed a unified framework for constructing summaries at multiple levels of granularity of a text document by employing a sequence-to-sequence network with attention in this work. The shortest summaries constructed this way are then expanded iteratively to generate summaries at subsequent granularity.    

\begin{comment}

\begin{figure}[t]
\includegraphics[width=0.95\linewidth]{plots/Fig2}
\centering
\caption{\label{fig:Picture2}\textbf{A bi-directional LSTM network pair is used to compute the minimal feasible summary of a document; At each timestep~$t$, the next token in the summary is generated by computing an weighted sum of attention distribution over the input text and the external vocabulary\looseness=-1}}\vspace{-0.5cm}
\end{figure}

\end{comment}

\textit{Incremental sampling: }In one of their early works, Otterbacher et al.~\cite{otterbacher2006news} proposed an incremental sampling based approach for summarizing documents at multiple budgets. Representing each document as a tree-like structure, sentences were sampled from each level to construct incrementally larger summaries. Campana et al.~\cite{campana2009incremental} followed a similar approach to generate personalized summaries by taking user-specific interactions into account. However, neither can generate summaries at arbitrary budgets.\looseness=-1\vspace{0.02cm} %MLS can be extended to complement such human-in-the-loop frameworks in the future.

\textit{
Length-constrained supervision: }Kikuchi et al.~\cite{kikuchi2016controlling} proposed were one of the earliest works to propose a supervised method for abstractive summarization at controllable budgets. Their work was later extended by Fan et al.~\cite{fan2017controllable} who incorporated length embeddings as additional inputs to a sequence-to-sequence network to construct summaries at specified budgets. However, they introduced a discretization step in their workflow that approximated the budget to a predefined value-range. Consequently, failing to adhere to the specified budget for a number of cases. Liu et al.~\cite{liu2018controlling} addressed this issue in their recent work. They introduced a convolutional approach that takes the desired length of a summary as an input to the initial state of the decoder to constrain the length of a summary. We compare against them in Section 4.\vspace{0.02cm}

\textit{Extract-then-compress:} Although not for budgeted summarization, prototype-text driven summarization has been investigated by previous researchers. In this method, once the most salient phrases of the input document (i.e., the \textit{prototype-text}) is extracted, the summary is constructed by rewriting or compressing the prototype-text using statistical models~\cite{jing2000cut,knight2000statistics}, integer linear programming~\cite{berg2011jointly}, or neural network models~\cite{cheng2016neural,chen2018fast}. These methods, however, do not construct budgeted summaries. We acknowledge the contemporary work by Saito et al.~\cite{saito2020length} to address this problem. To construct a budgeted summary, they extract the top-$K$ keywords of the input document. The final summary is constructed by expanding these keywords using an LSTM based encoder-decoder model. One of the major limitations of their work is finding the optimal value of~$K$, as setting it to a too small or high value may affect the quality of the final summaries. MLS avoids this issue by learning to infer the length of the minimal feasible summary (i.e. the prototype-text) from gold-standard summaries. We will show in Section 4 that the budgeted summaries constructed by MLS are coherent and complete.\looseness=-1\vspace{-0.15cm}
